Ultra-High-Frequency Harmony: mmWave Radar and Event Camera Orchestrate Accurate Drone Landing

For precise, efficient, and safe drone landings, ground platforms should real-time, accurately locate descending drones and guide them to designated spots. While mmWave sensing combined with cameras improves localization accuracy, the lower sampling frequency of traditional frame cameras compared to mmWave radar creates bottlenecks in system throughput. In this work, we replace the traditional frame camera with event camera, a novel sensor that harmonizes in sampling frequency with mmWave radar within the ground platform setup, and introduce mmE-Loc, a high-precision, low-latency ground localization system designed for drone landings. To fully leverage the \textit{temporal consistency} and \textit{spatial complementarity} between these modalities, we propose two innovative modules, \textit{consistency-instructed collaborative tracking} and \textit{graph-informed adaptive joint optimization}, for accurate drone measurement extraction and efficient sensor fusion. Extensive real-world experiments in landing scenarios from a leading drone delivery company demonstrate that mmE-Loc outperforms state-of-the-art methods in both localization accuracy and latency.

==> background.tex <==
% \& Motivation
% https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=6696456
\vspace{-0.3cm}
\section{Background}

\subsection{Delivery Drone Precise Landing Primer}
% The process of drone-based instant delivery operates as follows. 
% First, the package is manually placed on the drone. The drone then takes off from the departure platform located at the self-collection airport on top of the mall. It ascends to cruising altitude and navigates towards the designated destination, usually a self-collection station near the customer. As the drone nears the destination, it starts a precise landing sequence and begins its descent.
% Upon safely landing on the platform of the self-collection station, the drone releases the package into the station for customer retrieval. 
% The drone then departs and returns to the airport, landing on the landing platform of self-collection airport.
The process of drone-based instant delivery operates as follows:
$(i)$ The package is manually loaded onto the drone;
$(ii)$ The drone then takes off from the departure platform located at the self-collection airport usually on top of the mall;
$(iii)$ It ascends to cruising altitude and navigates toward the designated destination, typically a self-collection station near the customer;
$(iv)$ As the drone approaches the destination, it initiates a precise landing sequence and begins its descent;
$(v)$ Upon safely landing at the self-collection station, the drone releases the package for customer retrieval; 
$(vi)$ The drone then departs, returning to the self-collection airport and executing a precise landing on the landing platform.

% The consequences of not landing precisely cannot be overstated.
% Missing the platform can result in the drone losing control and crashing, risking damage or injury. 
% 控制Localization latency and localization error are vital to drone landing to avoid similar mishaps， as increased errors and delays in location updates can destabilize the system. 
% Specifically, significant localization latency provide the drone with minimal reaction time, and large localization errors can cause the flight controller to make incorrect maneuvers.
The importance of precise landing cannot be emphasized enough. 
Failing to land accurately can lead to the drone losing control and crashing, potentially causing harm or damage \cite{Russiandrone}. 
Minimizing localization error and latency is crucial for safe drone landing, as any increase in errors or delays in location updates can destabilize the system, leading to the failure happens. 
Specifically, reducing localization latency provides the drone with more reaction time, while minimizing localization errors prevents the flight controller from executing incorrect maneuvers.

% Instant delivery with a drone unfolds as follows. After the package通过人工的方式 is placed onboard , the drone takes off from departing platform of self-collection airport on the top of the mall, climbs to cruising altitude, and heads towards the destination. 
% The latter is typically a self-collection station near the customer. When the drone is close to the destination, a precise landing procedure is initiated, in which the drone starts the descent.
% Once the drone safely docks onto the landing platform of the self-collection station, the package is dropped into the self-collection station, where the customer fetches it.
% 随后，drone从self-collection station起飞，heading towards the airport and docks on the landing platform of self-collection airport.

% The consequences of not landing precisely can only be underestimated. 
% Loss of the transported good is the most obvious. Should the drone miss the landing platform even partly, it would quickly lose control and crash, possibly damaging objects or hurting people.
% Both the localization latency and localization error are crucial to drone landing, as evidence shows that increasing error of location estimation and latency of location updates represent sources of system instability.. 
% A long localization delay leaves the drone very short time to react, and a large localization error misleads the flight controller to execute a wrong maneuver.

%要不要加呢？？
% \subsection{Limitations of the Current Practice}
% \noindent \textbf{Examining the current practice.}
% During aerial navigation, the flight control system primarily utilizes GPS or RTK for location information. 
% As the drone descends, precise control according to location information is crucial to remain centered over the landing platform. 
% However, in environments like urban canyons, GPS or RTK accuracy may degrade, making them unreliable at lower altitudes where drone docking.
% To address this, auxiliary anchor-based systems like visual markers assist during descent.
% These markers are detected by downward-facing cameras on the drone. 
% However, as these methods rely on RGB cameras, their effectiveness is limited by camera inherent frame exposure time. 
% Additionally, factors like camera motion blurring, field of view and drone alignment may lead to incomplete marker capture, causing localization errors.
% Overall, existing methods fail to meet the requirements for localization accuracy and latency during the drone docking phase.

% \noindent \textbf{What is a feasible solution? } 
% As the drone descends to dock, achieving precise and low latency adjust based on localization result is crucial for accurate landing. 
% Thus, there are the key requirements in updating localization result for drones: 
% $(i)$ \textit{cm-level} localization accuracy and $(ii)$ \textit{ms-level} localization latency.


% \subsection{Fusing Event and mmWave: Opportunities and Challenges}
% \noindent $\bullet$ \textbf{C1: Noisy sensing results impairs drone detection and tracking.}
% Environmental changes often introduce irrelevant information in the sensing results from the event camera and mmWave radar, hindering the system's ability to identify signals changes caused by the drones to be tracked. 
% Additionally, modern flight control loops operate at frequencies exceeding 400 Hz, requiring the system to detect and track drones rapidly. 
% However, traditional noise filtering, object detection and tracking algorithms have high time complexities, resulting in precision and tracking frequency bottlenecks. 
% \todo{Explanation in figures or tables.}

% \noindent $\bullet$ \textbf{C2: Heterogeneous data fusion delays drone localization.}
% Once the drone is detected, accurate 3D spatial localization of it is essential, which is more time-consuming than detection and tracking due to additional processing. 
% Moreover, event cameras provide asynchronous event streams, while mmWave radar generates sparse point clouds with relatively low spatial resolution. 
% Previous fusion methods (\eg extended Kalman filters and particle filters) often suffer from significant cumulative drift error and lengthy processing times, rendering them inadequate for high-frequency and high-precision tracking.
% \todo{Explanation in figures or tables.}

\vspace{-0.3cm}
\subsection{HFPL: System goals}
HFPL takes a solid step forward in ensuring safely takeoff and landing of drone. 
We list the system goals below.

\noindent $\bullet$ \textbf{Goal 1: Low latency \& High precision localization.}
HFPL should provide low-latency and accurate localization results for the drone. This allows the drone's flight control loops to take advantage of HFPL and operate the drone to land at the designated location.\\
\noindent $\bullet$ \textbf{Goal 2: Plug and play.}
HFPL should be implemented as a plug-in module, seamlessly integrating with existing GPS/RTK and visual marker localization systems. This prevents deeply embedded code changes that could potentially compromise the system’s stability. \\
\noindent $\bullet$ \textbf{Goal 3: Resource overhead reduction.}
HFPL should effectively reduce the resource overhead spanning filtering and fusion for both sensing modalities, while maintaining the high-precision and low-latency performance.

==> intro.tex <==
% \vspace{-0.3cm}
\revise{\section{Introduction}}
% Drones have been one of the most disruptive inventions in recent years, giving rise to numerous innovative applications such as last-mile delivery, sky networking, and industrial inspection. 
% For example, in recent years, the roll-out of 5G networks in cities has made it possible for drones to perform beyond-line-of-sight operations and achieve instant asset delivery.
% Specifically, a drone can now fly autonomously to deliver goods over long distances without a human pilot on-site, while being monitored in real-time via an Internet-connected back-end system.
% The advantages of using drones for delivery are clear: drones can bypass complex urban traffic and deliver packages much faster, which is ideal for time-sensitive deliveries such as medical supplies. 
% Many companies are exploring the commercial feasibility of instant deliveries with drones, including Amazon, Alphabet's Project Wing, Walmart, JD.com, Domino’s, UPS, Ele.me, and Meituan.
% Drones have become one of the most disruptive inventions in recent years, leading to applications like last-mile delivery and industrial inspection. 
% For example, the roll-out of 5G networks in cities has enabled beyond-line-of-sight operations, allowing drones to deliver goods autonomously over long distances while being monitored in real-time. 
% These drones can bypass urban traffic, making them ideal for time-sensitive deliveries such as medical supplies. 
% Companies like Amazon, Alphabet's Project Wing, Walmart, JD.com, Domino’s, UPS, Ele.me, and Meituan are exploring the commercial potential of instant drone deliveries.
Drones have become one of the most disruptive technologies, with applications ranging from last-mile delivery \cite{floreano2015science} to industrial inspection \cite{bartolini2020multi}. 
The roll-out of 5G networks in cities enhances their capabilities, allowing drones to autonomously deliver goods over long distances while being monitored in real-time \cite{bertizzolo2021streaming}. 
Bypassing urban traffic, drones are especially effective for time-sensitive deliveries, such as medical supplies \cite{MedicalDelivery}. Various businesses, including Amazon \cite{Amazondrone}, Alphabet Wing \cite{Wingdrone}, and Meituan \cite{Meituandrone}, are exploring the viability of drones for instant deliveries, as shown in \fig \ref{intro}a.
% Drones have emerged as one of the most disruptive technologies in recent years \cite{floreano2015science}, with applications ranging from last-mile delivery\cite{xiang2021reusing} to industrial inspection \cite{bartolini2020multi}. 
% The roll-out of 5G networks in cities further enhances their capabilities, allowing drones to autonomously deliver goods over long distances while being monitored in real-time \cite{bertizzolo2021streaming}. 
% Bypassing urban traffic, drones are especially effective for time-sensitive deliveries (\eg medical supplies \cite{MedicalDelivery}).
% A variety of businesses are examining the viability of drones for instant deliveries, including Amazon\cite{Amazondrone}, Alphabet Wing\cite{Wingdrone}, Meituan\cite{Meituandrone}, as illustrated in \fig \ref{intro}a.

% Takeoff and landing are critical steps in the operation of a drone because during these stages, the drone is most vulnerable \cite{wang2022micnest, xu2023taming, zhao2023smoothlander}. 
% Specifically, the risk of damaging the drone or its surroundings is highest during these stages, which lead to financial losses and pose a threat to human safety, creating a significant barrier to the widespread adoption of drones\cite{Russiandrone}.
% Accurate and low-latency localization is crucial for the effective takeoff and landing of drones \cite{sun2023indoor}, as illustrated in \fig \ref{intro}b.
% Higher localization accuracy increases the likelihood of successful takeoff and landing on the designated platform, while lower localization latency provides more time for the drone to react to unexpected situations \cite{famili2022pilot, he2023acoustic, chi2022wi}. 

Takeoff and landing are critical phases in drone operation, requiring accurate, low-latency localization due to the heightened vulnerability of the drone during these stages , as shown in \fig \ref{intro}b \cite{wang2022micnest, zhao2023smoothlander, sun2023indoor}. 
During these phases, the risk of damage to the drone or its surroundings is elevated, potentially resulting in financial losses and posing safety risks, which hinder the widespread adoption of drones \cite{Russiandrone}. 
Enhanced localization accuracy improves the likelihood of successful takeoff and landing on the intended platform, while reduced localization latency allows the drone to respond more effectively to unexpected situations \cite{famili2022pilot, he2023acoustic, chi2022wi}. 

\begin{figure}[t]
    \setlength{\abovecaptionskip}{-0.2cm} % height above Figure X caption
    \setlength{\belowcaptionskip}{-0.24cm}
    \setlength{\subfigcapskip}{-0.25cm}
    \centering
        \includegraphics[width=1\columnwidth]{Figs/intro.png}
        \vspace{-0.2cm}
    \caption{Illustration of Delivery Drone.}
    \label{intro}
    \vspace{-0.4cm}
\end{figure} 



Unfortunately, current methods are not able to offer feasible solutions for accurate and low-latency localization of drone, which can be divided into two categories: \\
$\bullet$ \textbf{Extra infrastructure based solutions.} 
These solutions rely on external devices (\eg, GPS\cite{nirjon2014coin}, RTK\cite{wang2022micnest}, WiFi\cite{hu2023wisdom, chen2015drunkwalk}, microphone\cite{guo2021infrastructure, weiguo2020symphony}) to provide reference signals for localization, which require LoS connection between localization infrastructure and drones.
However, in densely built urban environments, the accuracy and environmental compatibility of these methods significantly degrades as altitude decreases, rendering ineffective for low-altitude operations \cite{li2021infocom_itoloc}. \\
$\bullet$ \textbf{Intra on-board sensor based solutions.}  
These solutions leverage onboard sensors (\eg, cameras\cite{xu2019ivr}, IMUs\cite{lu2020milliego}, lidar\cite{he2021vi} or radar\cite{dai2023interpersonal}), combined with simultaneous localization and mapping (SLAM) techniques\cite{campos2021orb} or visual markers\cite{krogius2019iros}, to achieve high-precision location estimation. 
% However, due to sensor performance limitations, these methods have significant localization latency, which is insufficient for the rapid localization requirements during drone landing \cite{xu2021followupar}.\\
However, the low spatio-temporal sampling resolution of these onboard sensors poses a challenge for drones to achieve timely and accurate localization during landing.\\
\textbf{Remark.} The absence of the efficient algorithms and sensors make it challenging for existing methods to achieve timely and accurate localization for drone, which requires $(i)$ $cm-level$ localization accuracy and $(ii)$ $ms-level$ localization latency to feed the control loop for effective takeoff and landing. \\
% Event cameras are innovative bio-inspired sensors that asynchronously report pixel-wise intensity changes. With microsecond resolution, they capture high-speed motions without blurring, making them ideal for tasks like high-speed feature and motion tracking.
% However, like RGB cameras, event cameras face scale uncertainty and cannot determine object depth, hindering accurate drone localization. 
% Current methods address this by integrating depth cameras or using dual event cameras. Yet, depth cameras' lower update frequency diminishes event cameras' advantages, and the significant noise in event cameras leads to lower-quality data and higher pose estimation errors.
% \begin{figure*}[t]
%     \setlength{\abovecaptionskip}{-0.1cm} % height above Figure X caption
%     \setlength{\belowcaptionskip}{-0.3cm}
%     \setlength{\subfigcapskip}{-0.25cm}
%     \centering
%         \includegraphics[width=2.1\columnwidth]{evaFigs/related.png}
%         \vspace{-0.2cm}
%     \caption{Principle of event camera and performance of existing solutions at different settings.}
%     \label{relatedwork}
%     \vspace{-0.2cm}
% \end{figure*} 

\begin{figure*}[t]
    \setlength{\abovecaptionskip}{0.2cm} % height above Figure X caption
    \setlength{\belowcaptionskip}{-0.3cm}
    \setlength{\subfigcapskip}{-0.25cm}
    \centering
        \includegraphics[width=2\columnwidth]{evaFigs/relatedall_2.png}
        % \vspace{-0.2cm}
    \caption{Benchmark study on drone localization and performance of existing solutions at different settings.}
    \label{relatedwork}
    % \vspace{-0.2cm}
\end{figure*} 

\noindent \textbf{Localization with event camera and mmWave radar.}
% Event cameras are bio-inspired sensors that asynchronously report pixel-wise intensity changes. With microsecond resolution, they capture high-speed motions without blurring, ideal for tasks like high-speed feature and motion tracking. However, like RGB cameras, they face scale uncertainty and cannot determine object depth, hindering accurate drone localization. Integrating depth cameras or using dual event cameras helps, but depth cameras' lower update frequency and event cameras' noise reduce data quality and increase pose estimation errors.
% We find that millimeter-wave (mmWave) radar, which can transmit and receive frequency-modulated continuous waves (FMCW) with ms-level latency, measuring the relative angle and distance of moving objects. 
% Both mmWave radar and event camera share ms-level time resolution, inspiring us to fuse them for high-accuracy, low-latency drone localization. 
% Event cameras are bio-inspired sensors that asynchronously report pixel-wise intensity changes with ms-level latency, capturing high-speed motions without blurring, ideal for tasks like feature and motion tracking. 
% However, similar to frame cameras, they struggle with scale uncertainty, hindering utilization in accurate drone localization. 
% Integrating depth cameras or using dual event cameras may help, but lower update frequency of depth cameras and noise of event cameras increase localization error and latency.
% Millimeter-wave (mmWave) radar, which transmits and receives frequency-modulated continuous waves (FMCW) with ms-level latency, measures the relative angle and distance of moving objects. 
% Both event camera and mmWave radar share ms-level time resolution, inspiring us to fuse them for high-accuracy, low-latency drone localization.
Event camera is bio-inspired sensor that report pixel-wise intensity changes with $ms-level$ latency \cite{xu2023taming}, capturing high-speed motions without blurring \cite{he2024microsaccade}, ideal for tasks like feature and motion tracking \cite{alzugaray2018asynchronous}.
% as shown in \fig \ref{relatedwork}a. 
However, they struggle with scale uncertainty, hindering accurate drone localization \cite{falanga2020dynamic}. 
Integrating depth cameras or using dual event cameras may help, but the lower update frequency of depth cameras and noise from event cameras increase localization latency and error \cite{he2021fast}. 
Millimeter-wave (mmWave) radar, utilizing frequency-modulated continuous waves (FMCW) with $ms-level$ latency, measures the relative angle and distance of moving objects \cite{woodford2023metasight, zheng2023neuroradar}. 
Both event camera and mmWave radar share $ms-level$ time resolution, inspiring us to fuse them for accurate, low-latency drone localization.
However, according to our benchmark study conducted with setup in \fig \ref{relatedwork}a, translating this intuition into a practical system is non-trivial and faces significant challenges:\\
% \noindent $\bullet$ \textbf{C1: Noisy sensing results impairs drone detection and tracking.}
% Environmental unexpected changes often introduce irrelevant information in the sensing results from the event camera and mmWave radar, hindering the system's ability to identify signals changes caused by the drones to be tracked, as shown in \fig \ref{relatedwork}b. 
% However, traditional noise filtering algorithms\cite{cao2024virteach, liu2024pmtrack, wang2021asynchronous, alzugaray2018asynchronous} achieve a low event and mmWave point cloud filtering rate (recall and precision < 65\% in \fig \ref{relatedwork}c) due to their rule-based pipelines, resulting in detection precision bottlenecks.
% Additionally, modern flight control loops operate at frequencies exceeding 400 Hz, requiring the system to filter the noise and track the drone rapidly. \\
\noindent $\bullet$ \textbf{C1: Noise distribution characteristics of both modalities differ, hindering drone detection.}
% Both sensor modalities yield not only heterogeneous information about the drone but also generate significantly heterogeneous noise. 
These two sensor modalities not only provide different types of information but also generate significantly heterogeneous noise. 
Event cameras produce noise due to unexpected changes in brightness conditions, whereas mmWave radar struggles with noise caused by signal multipath effects.
These noises differ greatly in both dimension and pattern, which can also be asynchronous, especially under high temporal resolution (\fig \ref{relatedwork}b).
This spatial and temporal heterogeneity complicates noise filtering, causing detection bottlenecks \cite{xu2023taming}.
Unfortunately, existing traditional noise filtering algorithms \cite{cao2024virteach, liu2024pmtrack, wang2021asynchronous, alzugaray2018asynchronous} typically target a single modality, resulting in low noise event and point cloud filtering rates (recall and precision < 65\% in \fig \ref{relatedwork}c), limiting their effectiveness in our scenario.\\
% \noindent $\bullet$ \textbf{C2: Heterogeneous data fusion delays drone localization.}
% Once the drone is detected, accurate 3D spatial localization of it is essential, which is more time-consuming than detection and tracking due to additional processing (\eg, feature matching). 
% As depicted in \fig \ref{relatedwork}d, although the localization accuracy is boosted, existing methods Baseline-I, -II and -III introduces significant delays, mismatching with flight control loops.
% Moreover, event cameras provide asynchronous event streams, while mmWave radar generates sparse point clouds with relatively low spatial resolution. 
% Previous fusion methods (\eg, extended Kalman filters and graph optimization in \fig \ref{relatedwork}d) often suffer from significant cumulative drift error and lengthy processing times, rendering them inadequate for accurate and low-latency localization.
\noindent $\bullet$ \textbf{C2: Ultra-large data volume burden the heterogeneous data fusion, delaying drone localization.}
Accurately estimating 3D location of the drone after detection involves time-consuming processing steps, such as sensor fusion and optimization. 
% Once the drone is detected, we proceed to perform 3D localization on it.
% Accurately estimating 3D spatial location of drone involves several time-consuming processing steps, including the sensor fusion and optimization.
The ultra-large amount of data due to the high frequency further exacerbates the processing time, causing significant delays \cite{xu2021followupar}.
Meanwhile, the asynchronous event streams and sparse point clouds are heterogeneous in terms of precision, scale, and density, add complexity the sensor fusion.
Existing methods (\eg, Extended kalman filter, particle filter, and graph optimization) suffer from cumulative drift error, heterogeneity issues and lengthy processing latency, rendering them inadequate for accurate and low-latency localization as shown in \fig \ref{relatedwork}d \cite{zhao20213d, falanga2020dynamic, mitrokhin2018event, grisetti2010tutorial}.

% \noindent \textbf{Our work.}
% In this work, we delve into the sensing principles of event camera and mmWave radar and propose HFPL, a system that provides $cm-level$ accurate drone localization with $ms-level$ latency. 
% HFPL features three key designs to fully harness the potential of events and mmWave point cloud for drone localization and is implemented with adaptively acceleration algorithms to further improve accuracy and reduce latency, as elaborated below: \\
% \noindent $\bullet$ \textit{On system architecture front.}
% By incorporating event camera and mmWave radar, sharing $ms-level$ time resolution, we improve drone localization accuracy and reduce latency at the data source.
% HFPL features a carefully designed system architecture that tightly couples event camera and mmWave radar. 
% This integration spans from early-stage filtering to later-stage fusion and optimization, fully extracting and leveraging the unique advantages of both sensors (§\ref{3.2}). \\
% \noindent $\bullet$ \textit{On system algorithm front.}
% We first introduce the Consi-stency-Instructed Collaborative Tracking (\textit{CCT}) algorithm to utilize the disparities in sensing principles of both modalities to filter out unexpected environment-triggered events and point clouds from a large volume of data with a low false positive rate, enhancing the tracking performance (§\ref{4.1}). 
% We then present the Graph-Informed Adaptive Joint Optimization (\textit{GAJO}) algorithm to fully fuse drone-related information from both modalities, reducing latency of the optimization in localizing the drone (§\ref{4.2}). \\
% \noindent $\bullet$ \textit{On system implementation front.}
% We further analyze the sources of latency and propose an Adaptive Optimization method for boosting the \textit{GAJO}. This method dynamically optimizes the set of locations rather than relying on a fixed sliding window, further enhancing the accuracy of localization and reducing latency (§\ref{5.1}).

% \noindent \textbf{Evaluation and Result.} 
% We fully implement HFPL with COTS mmWave radar and event camera and deploy it on drone landing platforms in both indoor and outdoor environments. 
% Extensive experiments are conducted with different flight conditions. 
% We compared the end-to-end drone localization accuracy and latency of HFPL with three SOTA methods.
% % $(i)$ a radar-based localization system \cite{zhao20213d}, $(ii)$ an event camera-based localization system \cite{falanga2020dynamic}, and $(iii)$ a dual camera-based localization system .
% % Over 30 hours of real-world experiments and 400GB of data collection, we show that HFPL meets the required standards, achieving a drone localization accuracy of \notice{xx} dm, outperforming the baselines by over \notice{xx\%}, a average latency of location update of \notice{xx} ms, suitable for flight control loops.
% Through over 30 hours of real-world experiments and 400GB of data collection, we demonstrate that HFPL meets the required standards. HFPL achieves a localization accuracy of 1.01 $dm$, surpassing all baselines by >50\%. HFPL further achieves localization latency of 5.15 $ms$, outperforming baselines by 50\% in average, suitable for flight control loops.
% Additionally, HFPL is shown to be marginally affected by factors such as drone type, velocity, and envir. conditions.\\
% \textbf{Real-world deployment.}
% We have deployed the sensing platform and HFPL at a real-world drone delivery airport as shown in \fig \ref{intro} to demonstrate usability of the system.
% 10 hours study shows that HFPL meets drone landing demands within the constraints of available resources.

% \begin{figure*}[t]
%     \setlength{\abovecaptionskip}{-0.1cm} % height above Figure X caption
%     \setlength{\belowcaptionskip}{-0.3cm}
%     \setlength{\subfigcapskip}{-0.25cm}
%     \centering
%         \includegraphics[width=2.1\columnwidth]{Figs/overview.png}
%         \vspace{-0.2cm}
%     \caption{System architecture of HFPL.}
%     \label{overview}
%     \vspace{-0.2cm}
% \end{figure*} 
\noindent \textbf{Our work.}
% We explore the sensing principles of the event camera and mmWave radar and propose EventLoc, an low latency-oriented event camera enhancement system that provides cm-level accurate 3D object localization with millisecond level latency to enable application of event camera in various 3D vision tasks.
We delve into the sensing principles of event cameras and mmWave radar, introducing EventLoc. 
This system enhances event camera functionality with a focus on low-latency drone localization, providing cm-level accuracy with millisecond latency in average. 
% As a result, EventLoc broadens event camera application in diverse 3D vision tasks.
In detail, EventLoc features three key designs to fully unleash the potential of event camera and mmWave radar for drone localization: \\
% and is implemented with adaptively acceleration algorithms to further improve accuracy and reduce latency, 
\noindent $\bullet$ \textbf{On system architecture front.}
By incorporating mmWave radar with millisecond latency, we enhance the performance of event camera and improve 3D localization performance at the data source.
EventLoc features a carefully designed system architecture that tightly couples event camera and mmWave radar. 
This integration spans from early-stage filtering to later-stage fusion and optimization, fully leveraging the unique advantages of both sensors (§\ref{3.2}). \\
\noindent $\bullet$ \textbf{On system algorithm front.}
We first introduce the Consi-stency-Instructed Collaborative Tracking (\textit{CCT}) algorithm to extract \textit{consistent information} in sensing data from both modalities to filter out environment-triggered noise with a low false positive rate, enhancing the detection performance with a low-latency (§\ref{4.1}). 
We then present the Graph-Informed Adaptive Joint Optimization (\textit{GAJO}) algorithm to fully fuse \textit{complementary information} from both modalities, accelerating the optimization in localizing the object (§\ref{4.2}). \\
\noindent $\bullet$ \textbf{On system implementation front.}
We further analyze the sources of latency and propose an Adaptive Optimization method for boosting the \textit{GAJO}. 
This method dynamically optimizes the set of locations rather than relying on a fixed sliding window, further enhancing the accuracy of localization and reducing latency (§\ref{5.1}).

\begin{figure*}[t]
    \setlength{\abovecaptionskip}{0.4cm} % height above Figure X caption
    \setlength{\belowcaptionskip}{-0.5cm}
    \setlength{\subfigcapskip}{-0.25cm}
    \centering
        \includegraphics[width=2\columnwidth]{Figs/overview2.png}
        \vspace{-0.2cm}
    \caption{System architecture of EventLoc.}
    \label{overview}
    % \vspace{-0.2cm}
\end{figure*} 

\noindent \textbf{Evaluation and Result.} 
We fully implement EventLoc with COTS event camera and mmWave radar.
Extensive experiments in indoor/outdoor environments are conducted with different drone flight conditions to comprehensively evaluate performance of EventLoc.
We compare the end-to-end drone localization accuracy and latency of EventLoc with three SOTA methods.
% Through over 30 hours of real-world experiments, we demonstrate that EventLoc enhances event camera with mmWave radar by achieving a localization accuracy of 1.01 $dm$, surpassing all baselines by >50\%. EventLoc further achieves localization latency of 5.15 $ms$, outperforming baselines by >50\% in average.
Through over 30 hours experiments, we demonstrate that EventLoc enhances event camera with mmWave radar by achieving a average localization accuracy of 0.101 $m$ and latency of 5.15 $ms$, surpassing all baselines by >50\% in average.
Additionally, EventLoc is marginally affected by factors such as drone type and envir. conditions.\\
\textbf{Real-world deployment.}
We have deployed the sensor platform with EventLoc at a real-world drone delivery airport as shown in \fig \ref{relatedwork}a to demonstrate practicability of the system.
10 hours study shows that EventLoc meets drone landing demands within the constraints of available resources.


% \noindent \textbf{Contributions.}
% \scalebox{1.2}{\ding{182}} We propose HFPL, a novel framework that tightly fuses asynchronous events and sparse point cloud to localize landing drone. HFPL can be integrated with existing GPS/RTK and visual marker to facilitate safe drone landing. 
% \scalebox{1.2}{\ding{183}} We propose the $CCT$, a light-weight cross-modal filter to push the limit of detection and tracking accuracy of drone by leveraging the differing trigger principles of the event camera and mmWave radar. 
% \scalebox{1.2}{\ding{184}} We design the $GAJO$, a factor graph-based optimization framework that fuses heterogeneous data to enhance localization accuracy and reduce latency by fully harnessing the potential of both modalities.
% \scalebox{1.2}{\ding{185}} We implement and extensively evaluate HFPL by comparing it with three SOTA methods. Evaluation results show the effectiveness of HFPL. We also deploy HFPL in a real-world drone delivery airport, demonstrating feasibility of HFPL.
\noindent \textbf{Contributions.} This paper makes following contributions.

\noindent $(1)$ We propose EventLoc, a novel low latency-oriented drone localization system. It tightly integrates asynchronous events and mmWave radar sparse point clouds, achieving accurate drone localization with millisecond latency.\\
\noindent $(2)$ We propose the $CCT$, a light-weight cross-modal noise filter to push the limit of detection accuracy by leveraging the \textit{consistent information} from both modalities. \\
\noindent $(3)$  We propose the $GAJO$, a factor graph-based optimization framework that fully harnessing \textit{complementary information} from both modalities to enhance localization performance.\\
% accuracy and latency
\noindent $(4)$ We implement and extensively evaluate EventLoc by comparing it with three SOTA methods, showing its effectiveness. We also deploy EventLoc in a real-world drone delivery airport, demonstrating feasibility of EventLoc.

==> intro1029.tex <==
% \vspace{-0.3cm}
\section{Introduction}
% Drones have become one of the most disruptive technologies, with applications ranging from last-mile delivery \cite{floreano2015science} to industrial inspection \cite{bartolini2020multi}. 
% The roll-out of 5G networks in cities enhances their capabilities, allowing drones to autonomously deliver goods over long distances while being monitored in real-time \cite{bertizzolo2021streaming}. 
% Bypassing urban traffic, drones are especially effective for time-sensitive deliveries, such as medical supplies \cite{MedicalDelivery}. Various businesses, including Amazon \cite{Amazondrone}, Alphabet Wing \cite{Wingdrone}, and Meituan \cite{Meituandrone}, are exploring the viability of drones for instant deliveries, as shown in \fig \ref{intro}a.
% Drones have emerged as a transformative technology in applications of last-mile delivery \cite{floreano2015science}. 
% Enabled by 5G, they can autonomously deliver goods over long distances, bypassing urban traffic—ideal for urgent needs like medical supplies \cite{MedicalDelivery}. 


Drones have become a transformative technology for last-mile delivery, with 5G enabling autonomous transport—ideal for urgent deliveries like medical supplies \cite{floreano2015science, MedicalDelivery}. 
A key phase in drone operation is landing, requiring active, accurate and low-latency localization from the ground due to the drone's increased vulnerability (\fig \ref{intro}a) \cite{wang2022micnest, zhao2023smoothlander, sun2023indoor}. 
Improved accuracy increases the chances of successful landing on target platforms, while lower latency enables faster responses to unforeseen situations \cite{famili2022pilot, he2023acoustic, chi2022wi} (\fig \ref{intro}b).
Mainstream ground-based systems leverage radar (\eg, mmWave radar) to achieve this goal, as it performs reliably across various lighting and noise conditions and offers a wide detection range \tocite.
% Currently ground-based practices primarily utilize radar (\eg, mmWave radar) to achieve active, accurate, low-latency localization for landing drone




% Currently ground-based practices primarily utilize radar (\eg, mmWave radar) to achieve active, accurate, low-latency localization for landing drone, which includes: 
Existing active, ground-based drone localization solutions utilizing mmWave radar fall into three categories:
% $(i)$ Introducing visual sensors, such as cameras, enables ground-based drone localization through multi-modal fusion. However, these methods increase system latency, as visual sensors require long frame exposure time and excessive image processing delay. Meanwhile, the motion blurring shown in each frame would confuse the localization algorithm, exacerbating localization errors.
% $(ii)$ \textit{conventional signal intensity-based methods}, however, challenge to accurately tracking drone's center due to its large size (\eg, 80 cm) and non-uniform blob radar readout. These methods also yield unstable results with frequent outliers, as noise or multipath scattering overpower the main signal.
$(i)$ \textit{conventional signal intensity-based methods}, however, struggle to accurately track the drone’s center due to its large size (\eg, 80$cm$ across), which cause the drone appears as a non-uniform blob in radar returns. These methods also yield unstable results with frequent outliers, as radar’s low spatial resolution and multipath scattering can overpower the main signal \tocite;
% $(ii)$ \textit{deep learning-based methods}, however, require extensive pre-modeling of the drone and prior neural network training. Meanwhile, These works can not track different models of drone.
$(iii)$ \textit{deep learning-based methods}, however, necessitate extensive pre-modeling of the drone and prior neural network training. These methods struggle to track different drone models and perform poorly in environments not represented in the training dataset \tocite. 
$(iii)$ \textit{Fusion-based methods} introduces visual sensors (\eg, cameras) to aid radar. However, these methods add system latency due to long exposure times (around 20$ms$) and additional image processing delays (another 10-20$ms$). Also, motion blur in frames can confuse the algorithm, increasing errors \tocite;\\
\textbf{Remark.} None of the previous solutions can achieve accurate, low-latency localization in diverse scenarios due to inefficient algorithms, environmental and drone-related uncertainties, and unsuitable sensor choices.

% $\bullet$ \textbf{Extra infrastructure based solutions.} 
% These solutions rely on external devices (\eg, GPS\cite{nirjon2014coin}, RTK\cite{wang2022micnest}, WiFi\cite{hu2023wisdom, chen2015drunkwalk}, microphone\cite{guo2021infrastructure, weiguo2020symphony}) to provide reference signals for localization, which require LoS connection between localization infrastructure and drones.
% However, in densely built urban environments, the accuracy and environmental compatibility of these methods significantly degrades as altitude decreases, rendering ineffective for low-altitude operations \cite{li2021infocom_itoloc}. \\
% $\bullet$ \textbf{Intra on-board sensor based solutions.}  
% These solutions leverage onboard sensors (\eg, cameras\cite{xu2019ivr}, IMUs\cite{lu2020milliego}, lidar\cite{he2021vi} or radar\cite{dai2023interpersonal}), combined with simultaneous localization and mapping (SLAM) techniques\cite{campos2021orb} or visual markers\cite{krogius2019iros}, to achieve high-precision location estimation. 
% However, the low spatio-temporal sampling resolution of these onboard sensors poses a challenge for drones to achieve timely and accurate localization during landing.\\
% \textbf{Remark.} The absence of the efficient algorithms and sensors make it challenging for existing methods to achieve timely and accurate localization for drone, which requires $(i)$ $cm-level$ localization accuracy and $(ii)$ $ms-level$ localization latency to feed the control loop for effective takeoff and landing. \\


\noindent \textbf{Enhance mmWave radars with event cameras.}
Event cameras are bio-inspired sensors that report pixel-wise intensity changes with $ms-level$ latency (\fig \ref{event}) \cite{xu2023taming}, capturing high-speed motions without blurring \cite{he2024microsaccade}, ideal for feature tracking tasks \cite{alzugaray2018asynchronous}.
% Event cameras share $ms-level$ time resolution with mmWave radar，and the 2D sensing capability of event cameras and the depth sensing capability of radar complement each other, inspiring us to enhance mmWave radar with event cameras for accurate, low-latency drone localization.
Event cameras also offer $ms-level$ time resolution consistent to radar, and their 2D sensing capability complements the limited spatial resolution of radar.
The both \textit{consistent} and \textit{complementary} information across both modalities inspiring us to enhance mmWave radar with event cameras for accurate, low-latency drone localization.

To explore the potential of this idea, we conduct a benchmark study on landing drone localization at a real-world drone delivery airport (\fig \ref{relatedwork}a). 
Our benchmark study reveals that translating this intuition into a practical localization system is non-trivial and faces significant challenges:\\
\noindent $\bullet$ \textit{C1: Noise distribution characteristics of both modalities differ, hindering drone detection.}
% Both sensor modalities yield not only heterogeneous information about the drone but also generate significantly heterogeneous noise. 
These two sensor modalities not only provide different types of information but also generate significantly heterogeneous noise. 
Event cameras produce noise due to unexpected changes in brightness conditions, whereas mmWave radar struggles with noise caused by signal multi-path effects.
These noises differ greatly in both dimension and pattern, which can also be asynchronous under high temporal resolution (\fig \ref{relatedwork}b).
This spatial and temporal heterogeneity complicates noise filtering, causing detection bottlenecks.
Existing noise filtering algorithms \cite{cao2024virteach, liu2024pmtrack, wang2021asynchronous, alzugaray2018asynchronous} \notice{chanage ref} typically target a single modality, resulting in low noise event and point cloud filtering rates (recall and precision < 65\% in \fig \ref{relatedwork}c), limiting their effectiveness.\\
\noindent $\bullet$ \textit{C2: Ultra-large data volume burden the heterogeneous data fusion, delaying drone localization.}
Accurately estimating 3D location of the drone after detection involves time-consuming sensor fusion and optimization. 
The ultra-large amount of data due to the high frequency further exacerbates the processing time, causing significant delays \cite{xu2021followupar}.
Meanwhile, the asynchronous event streams and radar readout are heterogeneous in terms of precision, scale, and density, add complexity to the sensor fusion.
Existing methods (\eg, Extended kalman filter and particle filter) suffer from cumulative drift error, heterogeneity issues and lengthy processing latency, rendering them inadequate for accurate and low-latency localization as shown in \fig \ref{relatedwork}d \cite{zhao20213d, falanga2020dynamic, mitrokhin2018event}. \notice{change ref in fig}

\begin{figure}[t]
    \setlength{\abovecaptionskip}{0.2cm} % height above Figure X caption
    \setlength{\belowcaptionskip}{-0.3cm}
    \setlength{\subfigcapskip}{-0.25cm}
    \centering
        \includegraphics[width=1\columnwidth]{Figs/event.png}
        \vspace{-0.5cm}
    \caption{Illustration of synchronous frames and asynchronous events. \textnormal{Frame cameras use a global shutter to output image frames at fixed intervals. In contrast, each pixel in an event camera responds independently and asynchronously, generating positive or negative events when intensity changes exceed a threshold.}}
    \label{event}
    \vspace{-0.4cm}
\end{figure} 

\noindent \textbf{Our work.}
We propose \textbf{EventLoc}, a robust, high-precision and low-latency landing drone localization system through enhancing mmWave radars functionality with event cameras.
% We delve into the sensing principles of event cameras and mmWave radar, introducing EventLoc. 
% This system enhances event camera functionality with a focus on low-latency drone localization, providing cm-level accuracy with millisecond latency in average. 
% As a result, EventLoc broadens event camera application in diverse 3D vision tasks.
EventLoc features three key designs to unleash the potential of mmWave radar and event camera for drone localization: \\
\noindent $\bullet$ \textbf{On system architecture front.}
% By incorporating event camera with $ms-level$ latency, we enhance the performance of mmWave radar and improve localization performance at the data source.
Incorporating an event camera with $ms-level$ latency enhances mmWave radar and improves localization at the data source.
% EventLoc features a carefully designed system architecture that tightly couples mmWave radar and event camera. 
% This integration spans from early-stage filtering to later-stage fusion and optimization, fully leveraging the unique advantages of both sensors (§\ref{3.2}). \\
The system architecture of EventLoc tightly integrates mmWave radar and the event camera, from early-stage filtering to later-stage fusion and optimization, fully leveraging the unique advantages of both sensors (§\ref{3.2}).\\
\noindent $\bullet$ \textbf{On system algorithm front.}
We first introduce a Consi-stency-Instructed Collaborative Tracking (\textit{CCT}) algorithm to extract \textit{consistent information} from both modalities to filter out environment-triggered noise with a low false positive rate, enhancing the detection performance with a low latency (§\ref{4.1}). 
We then present a Graph-Informed Adaptive Joint Optimization (\textit{GAJO}) algorithm to fully fuse \textit{complementary information}, accelerating the optimization (§\ref{4.2}). \\
\noindent $\bullet$ \textbf{On system implementation front.}
We further analyze the sources of latency and propose an Adaptive Optimization method for boosting the \textit{GAJO}. 
This method dynamically optimizes the set of locations, further enhancing the accuracy of localization and reducing latency (§\ref{5.1}).
\begin{figure}[t]
    \setlength{\abovecaptionskip}{0.2cm} % height above Figure X caption
    \setlength{\belowcaptionskip}{-0.3cm}
    \setlength{\subfigcapskip}{-0.25cm}
    \centering
        \includegraphics[width=1\columnwidth]{Figs/relatedall_3.png}
        \vspace{-0.5cm}
    \caption{Benchmark study on drone localization and performance of existing solutions at different settings.}
    \label{relatedwork}
    \vspace{-0.4cm}
\end{figure} 


\begin{figure*}[t]
    \setlength{\abovecaptionskip}{0.4cm} % height above Figure X caption
    \setlength{\belowcaptionskip}{-0.5cm}
    \setlength{\subfigcapskip}{-0.25cm}
    \centering
        \includegraphics[width=2\columnwidth]{Figs/overview2.png}
        \vspace{-0.2cm}
    \caption{System architecture of EventLoc.}
    \label{overview}
    % \vspace{-0.2cm}
\end{figure*} 




% \noindent \textbf{Evaluation and Result.} 
% We fully implement EventLoc with COTS event camera and mmWave radar.
% Extensive experiments in indoor/outdoor environments are conducted with different drone flight conditions to comprehensively evaluate performance of EventLoc.
% We compare the end-to-end drone localization accuracy and latency of EventLoc with three SOTA methods.
% Through over 30 hours experiments, we demonstrate that EventLoc enhances event camera with mmWave radar by achieving a average localization accuracy of 0.101 $m$ and latency of 5.15 $ms$, surpassing all baselines by >50\% in average.
% Additionally, EventLoc is marginally affected by factors such as drone type and envir. conditions.\\
% \textbf{Real-world deployment.}
% We have deployed the sensor platform with EventLoc at a real-world drone delivery airport as shown in \fig \ref{relatedwork}a to demonstrate practicability of the system.
% 10 hours study shows that EventLoc meets drone landing demands within the constraints of available resources.
\noindent \textbf{Evaluation and Results.}  
We fully implement EventLoc using COTS event cameras and mmWave radar. 
Comprehensive indoor and outdoor experiments under various drone flight conditions assess its localization accuracy and end-to-end latency performance against three SOTA methods.
Over 30+ hours of testing, EventLoc achieves an average localization accuracy of 0.101 m and latency of 5.15 ms, surpassing baselines by over 50\% and showing minimal sensitivity to drone type and environment.
% \textbf{Real-World Deployment.}  
We also deploy EventLoc at a real-world drone delivery airport (\fig \ref{relatedwork}a), demonstrating its practicality. A 10-hour study confirms EventLoc meets drone landing requirements within resource limits.
 
In summary, this paper makes following contributions.\\
\noindent $(1)$ We propose EventLoc, a active, contactless, ground-based, low latency-oriented landing drone localization system. 
It enhance the mmWave radar with asynchronous events, achieving accurate drone localization with millisecond latency. \\
% It tightly integrates asynchronous events and mmWave radar sparse point clouds, achieving accurate drone localization with millisecond latency.\\
\noindent $(2)$ We propose the $CCT$, a light-weight cross-modal noise filter to push the limit of detection accuracy by leveraging the \textit{consistent information} from both modalities. \\
\noindent $(3)$  We propose the $GAJO$, a factor graph-based optimization framework that fully harnessing \textit{complementary information} from both modalities to enhance localization performance.\\
% accuracy and latency
\noindent $(4)$ We implement and extensively evaluate EventLoc by comparing it with three SOTA methods, showing its effectiveness. We also deploy EventLoc in a real-world drone delivery airport, demonstrating feasibility of EventLoc.

==> intro_cxc.tex <==
\vspace{-0.5cm} 
\section{Introduction}

Event cameras are innovative bio-inspired sensors that asynchronously report pixel intensity changes as events with \textit{millisecond latency} (\fig \ref{intro}a), instead of fixed interval frames \cite{he2024microsaccade, gehrig2024low}.  
With high temporal resolution and a high dynamic range, event cameras excel at capturing high-speed motions without blurring and perform well under varied illumination conditions \cite{falanga2020dynamic, xu2023taming}.
Thus, event cameras are envisioned as an ideal solution for 2D vision tasks (\eg, low latency and accurate object detection in \fig \ref{intro}b \cite{gallego2020event}).

Although event cameras excel in 2D vision tasks, they face fundamental challenges in 3D vision, preventing their full potential from being realized.
Specifically, 3D object localization, identifying the location of objects within the camera's field of view in three dimensions, is a fundamental function for various vital 3D vision tasks (\eg, drone localization \cite{wang2022micnest}, AR/MR \cite{xu2021followupar}).
However, event cameras, capturing only 2D images without depth details, can't directly gauge object distance, causing scale uncertainty. 

This limitation restricts event cameras in 3D object localization (\fig \ref{intro}c), hindering the exploitation of their low-latency advantage in 3D vision tasks.
To address this, two types of solutions are proposed:


\noindent $\bullet$ \textbf{Events only-based solutions.}
These methods solely utilize event data for object depth estimation and fall into two types. 
$(i)$ Incorporating known geometric information with observations to deduce depth relies heavily on prior knowledge, leading to poor performance in new scenes or with new objects \cite{falanga2020dynamic}.
$(ii)$ These methods involves machine learning algorithms, which either stick events within a time window (\eg, $1ms$) into an image for DNN-based estimation \cite{guo2022low}, or devise event-oriented networks (\eg, SNN \cite{zhou2023computational}) for object localization \cite{barchid2023spiking}. 
However, they often entail significant delays (\eg, tens to hundreds of milliseconds) for network inference \cite{diehl2015unsupervised, guo2021toward}, negating low-latency benefits of event cameras.

\noindent $\bullet$ \textbf{Fusion-based solutions.}
These methods enhance event cameras for 3D object localization through sensor fusion, categorized into two types.
$(i)$ Several practices involve dual event cameras \cite{zhou2021event, xu2023taming}. 
% for 3D object localization
However, they often require meticulous calibration and feature matching between cameras, which are time-consuming and sensitive to environmental noise \cite{falanga2020dynamic}.
$(ii)$ Introducing dedicated depth estimation sensors (\eg, depth cameras \cite{he2021fast}, LiDAR \cite{cui2022dense}) provides event cameras with depth of objects \cite{li2022motion}. 
However, these sensors typically operate with sensing latency of 30$ms$ $\sim$ 100$ms$ \cite{li2023leovr}, requiring downsampling event cameras to synchronize, which nullify the low-latency benefits of event cameras.

\noindent \textbf{Remark.}
Inappropriate sensor choice for fusion and the absence of suitable algorithms negate the low-latency advantages of event cameras, posing challenges in fully leveraging their potential for low-latency 3D object localization.

\begin{figure}[t]
    \setlength{\abovecaptionskip}{0.25cm} % height above Figure X caption
    \setlength{\belowcaptionskip}{-0.3cm}
    \setlength{\subfigcapskip}{-0.25cm}
    \centering
        \includegraphics[width=0.98\columnwidth]{Figs/intro_new.png}
        \vspace{-0.2cm}
    \caption{Illustration of events generation and applications of event cameras.}
    \label{intro}
    \vspace{-0.3cm}
\end{figure} 

\begin{figure*}[t]
    \setlength{\abovecaptionskip}{0.2cm} % height above Figure X caption
    \setlength{\belowcaptionskip}{-0.3cm}
    \setlength{\subfigcapskip}{-0.25cm}
    \centering
        \includegraphics[width=2\columnwidth]{evaFigs/relatedall_2.png}
        \vspace{-0.2cm}
    \caption{Benchmark study on drone localization and performance of existing solutions at different settings.}
    \label{relatedwork}
    \vspace{-0.2cm}
\end{figure*} 

\noindent \textbf{Enhance event camera with mmWave radar.}
mmWave signals, operating at high frequencies (30 $\sim$ 300 GHz) with wide bandwidth, offer high sensing sensitivity and precision \cite{fiandrino2019scaling, zhang2023survey}.
Endowed with fine-grained, directional sensing capability, and resistance to weather and illumination conditions, mmWave sensing has great advantages in object depth estimation \cite{sie2023batmobility, iizuka2023millisign, lu2020see, lu2020milliego}.
More importantly, both event cameras and mmWave radar share \textit{millisecond latency} \cite{mmWaveUser}. These factors make mmWave a promising enhancement for event cameras in low-latency 3D object localization.

To explore the potential of fusing the event camera and mmWave radar for low-latency and accurate 3D object localization, we conduct a benchmark study on drone localization at landing phase at a real-world drone delivery airport (\fig \ref{relatedwork}a). 
Low-latency and accurate localization is crucial for effective landing of the drone \cite{wang2022micnest, sun2023indoor}, as in this phase the drone is most vulnerable \cite{xu2023taming, floreano2015science}, posing financial risks and safety threats \cite{Russiandrone}. 
Enhanced accuracy improves landing success on designated platforms, while reduced latency provides more reaction time for unexpected situations \cite{famili2022pilot, he2023acoustic, chi2022wi}.
Our benchmark study reveals that this fusion faces fundamental challenges in 3D object localization, as elaborated below:
 
\noindent $\bullet$ \textbf{C1: Differing noise distribution characteristics of both modalities hinder drone detection.}
Both sensor modalities yield not only heterogeneous information about the drone but also generate significantly heterogeneous noise. 
Event cameras produce noise due to unexpected changes in brightness conditions, while mmWave radar struggles with noise caused by signal multipath effects.
This noise differs greatly in dimensions and patterns, and it may lacks temporal synchronization, particularly under millisecond latency (\fig \ref{relatedwork}b). 
These factors make noise filtering challenging, causing detection bottlenecks and reducing localization efficiency and accuracy \cite{xu2023taming}.
Traditional noise filtering algorithms \cite{cao2024virteach, liu2024pmtrack, wang2021asynchronous, alzugaray2018asynchronous} target a specific modality, resulting in low noise event and point cloud filtering rates (recall and precision < 65\% in \fig \ref{relatedwork}c), limiting their effectiveness in our scenario.


\noindent $\bullet$ \textbf{C2: Ultra-large amount data burden the heterogeneous data fusion, delaying drone localization.}
Once the drone is detected, accurate 3D spatial location estimation of it is essential, which is more time-consuming than detection due to additional processing (\eg, sensor fusion and optimization).
The ultra-large amount of data generated by the millisecond latency further burdens the time consumption \cite{xu2021followupar}. 
Although the localization accuracy is boosted, existing methods \cite{zhao20213d, falanga2020dynamic, mitrokhin2018event} introduces significant delays (\fig \ref{relatedwork}d).
Moreover, asynchronous event streams and sparse point clouds from mmWave radar are heterogeneous in terms of precision, scale, and density. 
Previous fusion methods (\eg, Extended kalman filter, particle filter, and graph optimization \cite{grisetti2010tutorial} in \fig \ref{relatedwork}d) suffer from severe cumulative drift error and lengthy processing latency, rendering them inadequate for accurate and low-latency localization.

\noindent \textbf{Our work.}
We delve into the sensing principles of event cameras and mmWave radar, introducing EventLoc. This system, focused on low-latency, enhances event camera functionality, providing cm-level 3D object localization with millisecond latency in average, broadening its application in diverse 3D vision tasks.
EventLoc features three key designs to fully unleash the potential of event camera and mmWave radar for 3D object localization, as elaborated below: \\
\noindent $\bullet$ \textbf{On system architecture front.}
By incorporating mmWave radar with millisecond latency, we enhance the performance of event camera and improve 3D localization performance at the data source.
EventLoc features a carefully designed system architecture that tightly couples event camera and mmWave radar. 
This integration spans from early-stage filtering to later-stage fusion and optimization, fully leveraging the unique advantages of both sensors (§\ref{3.2}). \\
\noindent $\bullet$ \textbf{On system algorithm front.}
We first introduce the Consi-stency-Instructed Collaborative Tracking (\textit{CCT}) algorithm to extract \textit{consistent information} in sensing data from both modalities to filter out environment-triggered noise with a low false positive rate, enhancing the detection performance with a low-latency (§\ref{4.1}). 
We then present the Graph-Informed Adaptive Joint Optimization (\textit{GAJO}) algorithm to fully fuse \textit{complementary information} from both modalities, accelerating the optimization in localizing the object (§\ref{4.2}). \\
\noindent $\bullet$ \textbf{On system implementation front.}
We further analyze the sources of latency and propose an Adaptive Optimization method for boosting the \textit{GAJO}. 
This method dynamically optimizes the set of locations rather than relying on a fixed sliding window, further enhancing the accuracy of localization and reducing latency (§\ref{5.1}).

\begin{figure*}[t]
    \setlength{\abovecaptionskip}{0.4cm} % height above Figure X caption
    \setlength{\belowcaptionskip}{-0.5cm}
    \setlength{\subfigcapskip}{-0.25cm}
    \centering
        \includegraphics[width=2\columnwidth]{Figs/overview2.png}
        \vspace{-0.2cm}
    \caption{System architecture of EventLoc.}
    \label{overview}
    % \vspace{-0.2cm}
\end{figure*} 

\noindent \textbf{Evaluation and Result.} 
We fully implement EventLoc with COTS event camera and mmWave radar.
Extensive experiments in indoor/outdoor environments are conducted with different drone flight conditions to comprehensively evaluate performance of EventLoc.
We compare the end-to-end drone localization accuracy and latency of EventLoc with three SOTA methods.
Through over 30 hours experiments, we demonstrate that EventLoc enhances event camera with mmWave radar by achieving a average localization accuracy of 0.101 $m$ and latency of 5.15 $ms$, surpassing all baselines by >50\% in average.
Additionally, EventLoc is marginally affected by factors such as drone type and envir. conditions.\\
\textbf{Real-world deployment.}
We have deployed the sensor platform with EventLoc at a real-world drone delivery airport as shown in \fig \ref{relatedwork}a to demonstrate practicability of the system.
10 hours study shows that EventLoc meets drone landing demands within the constraints of available resources.

\noindent \textbf{Contributions.} This paper makes following contributions.

\noindent $(1)$ We propose EventLoc, a novel low latency-oriented event camera enhancement system. It tightly integrates asynchronous events and mmWave radar sparse point clouds, achieving accurate drone localization with millisecond latency.\\
\noindent $(2)$ We propose the $CCT$, a light-weight cross-modal noise filter to push the limit of detection accuracy by leveraging the \textit{consistent information} from both modalities. \\
\noindent $(3)$  We propose the $GAJO$, a factor graph-based optimization framework that fully harnessing \textit{complementary information} from both modalities to enhance localization performance.\\
\noindent $(4)$ We implement and extensively evaluate EventLoc by comparing it with three SOTA methods, showing its effectiveness. We also deploy EventLoc in a real-world drone delivery airport, demonstrating feasibility of EventLoc.



==> intro_new.tex <==
\vspace{-0.5cm} 
\section{Introduction}
% Event cameras are innovative bio-inspired sensors.
% Unlike traditional frame cameras, Event cameras do not operate at a fixed rate but asynchronously report pixel-wise intensity changes, known as events (\fig \ref{relatedwork}a). 
% With microsecond level resolution and an asynchronous, differential operating principle, event cameras excel at capturing high-speed motions that cause severe motion blur in frame cameras. 
% Additionally, Event cameras have a very high dynamic range (HDR) of 140dB compared to 60dB in frame cameras, performing well under varied illumination conditions. 
% Consequently, event cameras are considered an important sensing modality and are increasingly used for tasks like motion tracking and Simultaneous Localization and Mapping (SLAM).


% Event cameras are innovative bio-inspired sensors that report pixel-wise intensity changes as events asynchronously with microsecond sensing latency (\fig \ref{intro}a), rather than fixed interval frames \tocite. sensing latency is the time from a visual stimulus appearing to its sensor readout.
% Event cameras are innovative bio-inspired sensors that asynchronously report pixel brightness changes as events with \textit{millisecond latency} (\fig \ref{intro}a), instead of fixed interval frames \cite{he2024microsaccade, gehrig2024low}.  
% % sensing latency is the time from visual stimulus to sensor readout \cite{gehrig2024low}.
% With high temporal resolution and a high dynamic range, event cameras excel at capturing high-speed motions without blurring and perform well under varied illumination conditions \cite{falanga2020dynamic, xu2023taming}.
% Thus, event cameras are envisioned as an ideal solution for challenging 2D vision tasks, such as low latency and accurate object detection in \fig \ref{intro}b \cite{gallego2020event}.

Event cameras are innovative bio-inspired sensors that report changes in pixel brightness asynchronously as events with \textit{millisecond latency} (\fig \ref{intro}a), rather than at fixed-time
intervals \cite{he2024microsaccade, gehrig2024low}.  
% sensing latency is the time from visual stimulus to sensor readout \cite{gehrig2024low}.
With high temporal resolution and a high dynamic range, event cameras excel at capturing high-speed motions without blurring and perform well under varied illumination conditions \cite{falanga2020dynamic, xu2023taming}.
Thus, event cameras are envisioned as an ideal solution for 2D vision tasks, such as low latency and accurate object detection as shown in \fig \ref{intro}b \cite{gallego2020event}.

% Similar to frame cameras, event cameras encounter scale uncertainty (\aka, they struggle to accurately estimate object depth) \tocite.
% This challenge hinders event cameras from fully realizing their potential in 3D object localization \tocite. 
% Similar to frame cameras, event cameras encounter scale uncertainty (\aka, they struggle to accurately estimate object depth) \tocite.
% This challenge hinders event cameras from fully realizing their potential in 3D object localization \tocite. 
% 尽管事件相机在上述 2D vision tasks取得了不错的表现，
% However, event cameras struggle to fully realize their potential in low-latency 3D object localization, which has various potential applications (\eg, drone localization，入侵物体定位等）
% because they encounter scale uncertainty (\aka, they struggle to accurately estimate depth) \cite{zhang2022mobidepth}. 
% Although event cameras perform well in the aforementioned 2D vision tasks, they struggle to fully realize their potential in low-latency 3D object localization, which 对事件相机视野中出现的物体进行三维定位， has various potential applications (\eg, drone localization, intruding object detection, AR/MR) due to scale uncertainty (\aka, difficulty in accurately estimating depth) \cite{zhang2022mobidepth}.
% Although event cameras excel in the 2D vision tasks, they struggle to fully realize their potential in 3D vision tasks 以 low-latency 3D object localization为代表, which involves localizing the object within the camera's field of view in three dimensions (\fig \ref{intro}c). 
% Although event cameras excel in aforementioned 2D vision tasks, they struggle to fully realize their potential in 3D vision tasks, particularly in low-latency 3D object localization, which involves localizing objects within the camera's field of view in three dimensions (\fig \ref{intro}c) \cite{qin2019monogrnet}.
% The latency measures the time elapsed from visual stimulus to resulting localization output.
% This limitation, due to scale uncertainty (\ie, difficulty in accurately estimating depth) \cite{zhang2022mobidepth}, affects various potential vital applications of event cameras (\eg, drone localization \cite{wang2022micnest}, intruding object detection\cite{han2015twins}).

% Although event cameras excel in 2D vision tasks, they face fundamental challenges in 3D vision, preventing their full potential from being realized.
% Specifically, 3D object localization, identifying the location of objects within the camera's field of view in three dimensions, is a fundamental function for various vital 3D vision tasks (\eg, drone localization \cite{wang2022micnest}, AR/MR \cite{xu2021followupar}).
% However, event cameras, capturing per-pixel brightness changes in 2D without depth details, can't directly gauge object distance, causing scale uncertainty. 
% This limitation restricts event cameras in 3D object localization , hindering the exploitation of their low-latency advantage in 3D vision tasks.
% % To address this, 
% Two types of solutions are proposed:

However, event cameras face significant challenges when applied to more complex 3D vision tasks.
% which prevents their full potential from being realized. 
For instance, 3D object localization, which identifies the location of objects within the camera's field of view in three dimensions, is a fundamental block for various vital 3D vision tasks (\eg, drone navigation \cite{wang2022micnest}, augmented/mixed reality \cite{xu2021followupar}).
Event cameras only capture per-pixel brightness changes in 2D devoid of depth details, resulting in scale uncertainty that hinders their effectiveness in 3D object localization (\fig \ref{intro}c).
This limitation further restricts the exploitation of their potential in various 3D vision tasks.
To address this, two primary types of solutions are proposed to enhance event cameras:

% However, event cameras can only capture 2D images and lack depth information, making it impossible to directly measure the actual distance of the object. 
% This leads to scale uncertainty, preventing event cameras from performing 3D object localization (\fig \ref{intro}c).
% This prevents 3D object localization from leveraging the low-latency advantage of event cameras and hinders their use in various vital 3D vision applications.
% Two type solutions are proposed to augment event cameras:

% However, similar to frame cameras, event cameras face scale uncertainty (\aka, they cannot accurately estimate the depth of objects) \tocite.
% This is a fundamental challenge that prevents event cameras from fully realizing their potential in 3D object localization and tracking \tocite. 
% There are mainly two types of solutions proposed to address this issue, supplementing event cameras with depth information of objects:

\noindent $\bullet$ \textbf{Events only-based solutions.}
These methods rely solely on event data for object depth estimation and fall into two types. 
$(i)$ Incorporating known geometric information with observations to deduce depth. 
These methods rely heavily on prior knowledge, leading to poor performance in new scenes or with new objects \cite{falanga2020dynamic}.
$(ii)$ Employing machine learning algorithms that either stick events within a time window (\eg, $1ms$) into an image for DNN-based estimation \cite{guo2022low}, or devise event-oriented networks (\eg, SNN) for object localization \cite{zhou2023computational, barchid2023spiking}. 
These methods are computationally intensive during network inference \cite{diehl2015unsupervised, guo2021toward}, potentially entailing significant latency (\eg, tens to hundreds of milliseconds) in practice.

% However, they often entail significant delays (\eg, tens to hundreds of milliseconds) for network inference \cite{diehl2015unsupervised, guo2021toward}, negating low-latency benefits of event cameras.

% CNNs struggle to process event data directly due to its asynchronous nature \tocite. 
% Current practices

% These methods use only event data for object depth estimation, which can be categorized into two types.
% One type is machine learning algorithms. 
% Convolutional neural networks (CNNs) cannot directly process event data due to its asynchronous nature \tocite. 
% Current methods either stick events within a short time window (\eg, $<1ms$) into an image for CNN-based depth estimation \tocite or design event-oriented networks (\eg, spiking neural networks) for object localization \tocite. 
% However, these methods often require significant delays (\eg, tens to hundreds of milliseconds) for inference \cite{diehl2015unsupervised, guo2021toward}, negating the low-latency benefits of event cameras\tocite.
% The other type of methods incorporates known geometric information of the target object combined with observational data to infer depth, which heavily rely on prior knowledge, resulting in poor performance in new scenes and with unfamiliar objects.

\noindent $\bullet$ \textbf{Fusion-based solutions.}
These methods enhance event cameras for 3D object localization through sensor fusion, categorized into two types.
$(i)$ Involving dual event cameras \cite{zhou2021event, xu2023taming}. 
These methods often require meticulous calibration and feature matching between event cameras, which are time-consuming and sensitive to environmental noise \cite{falanga2020dynamic}.
$(ii)$ Introducing dedicated depth estimation sensors (\eg, depth cameras \cite{he2021fast}, LiDAR \cite{cui2022dense}) to provide event cameras with depth information \cite{li2022motion}. 
% However, these sensors typically operate at 10$Hz$ $\sim$ 30$Hz$ \tocite, requiring downsampling event cameras to synchronize, which nullify the low-latency benefits of event cameras \tocite.
However, these sensors typically operate with latencies ranging from 30$ms$ to 100$ms$ \cite{li2023leovr}, necessitating the downsampling of event data in the temporal domain for synchronization.
% requiring downsampling event cameras to synchronize, which nullify the low-latency benefits of event cameras.

\noindent \textbf{Remark.}
% In summary, current methods entail lengthy processing times or necessitate downsampling event cameras for synchronization with other sensors, presenting significant challenges in fully harnessing the potential of event cameras for low-latency 3D object localization.
% Inappropriate sensor choice for fusion and the absence of suitable algorithms negate the low-latency advantages of event cameras, posing challenges in fully leveraging their potential for low-latency 3D object localization.
In summary, the absence of efficient algorithms and the sensor with matched frequencies for depth estimation introduces substantial delays in 3D object localization. 
This limitation prevents the complete exploitation of the low-latency benefits of event cameras.

% "In summary, the lack of efficient algorithms and appropriately synchronized sensors for depth estimation causes significant delays in 3D object localization. This hurdle hinders the complete exploitation of the low-latency advantages offered by event cameras."
% event cameras’ potential.

% \noindent $\bullet$ \textbf{Dedicated depth sensors-based solution.}
% By introducing dedicated depth estimation sensors (\eg, depth cameras and LiDAR), these solutions provide event cameras with depth information of objects. 
% Specifically, these sensors emit light in a specific spectrum and calculate depth based on reflection time.
% However, they typically operate at frequencies of 10Hz $\sim$ 30Hz, much lower than the sampling frequency of event cameras, degrading localization performance.

% \noindent $\bullet$ \textbf{Learning-based solution.}
% Machine learning algorithms, such as convolutional neural networks (CNNs), cannot directly process event camera data because it consists of asynchronous events, not fixed-rate frames. 
% Current practices either $(i)$ stick all events within a short time window (\eg, $<1ms$) into an image for CNN-based depth estimation, or $(ii)$ design event-oriented networks (\eg, spiking neural networks) for object localization. 
% They rely heavily on labeled training data, leading to poor performance with new scenes and objects. Also, they introduce significant delays, negating the low-latency benefits of event cameras.

% \noindent $\bullet$ \textbf{Motion-based solution.}
% These methods combine information from inertial measurement units (IMUs) and use visual-inertial odometry to estimate 3D location of the target object. 
% Although they do not rely on dedicated sensors or training data, they require camera movement while the object remains stationary, which severely limits usage scenarios. 
% Additionally, current practices involve using dual event cameras with known pose relationships for 3D object localization. 
% However, these methods often require meticulous calibration and feature matching between cameras, which are highly sensitive to unexpected noise in the environment.

\begin{figure}[t]
    \setlength{\abovecaptionskip}{0.25cm} % height above Figure X caption
    \setlength{\belowcaptionskip}{-0.3cm}
    \setlength{\subfigcapskip}{-0.25cm}
    \centering
        \includegraphics[width=0.98\columnwidth]{Figs/intro_new.png}
        \vspace{-0.2cm}
    \caption{Illustration of events generation and applications of event cameras.}
    \label{intro}
    \vspace{-0.3cm}
\end{figure} 

\begin{figure*}[t]
    \setlength{\abovecaptionskip}{0.2cm} % height above Figure X caption
    \setlength{\belowcaptionskip}{-0.3cm}
    \setlength{\subfigcapskip}{-0.25cm}
    \centering
        \includegraphics[width=2\columnwidth]{evaFigs/relatedall_2.png}
        \vspace{-0.2cm}
    \caption{Benchmark study on drone localization and performance of existing solutions at different settings.}
    \label{relatedwork}
    \vspace{-0.2cm}
\end{figure*} 

\noindent \textbf{Enhance event camera with mmWave radar.}
% MmWave radar, utilizing frequency-modulated continuous waves (FM-CW) with microsecond level latency, measures relative angle and distance of moving objects, generating sparse point cloud \cite{woodford2023metasight, zheng2023neuroradar}. 
% with microsecond level latency
% MmWave radar, utilizing frequency-modulated continuous waves (FM-CW), has been widely employed to measure the relative angle and distance of moving objects, resulting in a sparse point cloud \cite{woodford2023metasight, zheng2023neuroradar}.
% The mmWave radar, utilizing frequency-modulated continuous waves (FM-CW), has been widely employed in detection and tracking of moving objects, resulting in a sparse point cloud \cite{woodford2023metasight, zheng2023neuroradar}.
% Inspired by achievements of mmWave-based sensing techniques, we observe that both event camera and mmWave radar share microsecond time resolution, making mmWave radar a promising modality to enhance the event camera in 3D object localization.
% This presents a significant opportunity for event-based accurate and low-latency localization.
mmWave signals, operating at high frequencies (30 $\sim$ 300 GHz) with wide bandwidth, offer high sensing sensitivity and precision \cite{fiandrino2019scaling, zhang2023survey}.
Endowed with fine-grained, directional sensing capability, and resistance to weather and illumination conditions, mmWave sensing has great advantages in object depth estimation \cite{sie2023batmobility, iizuka2023millisign, lu2020see, lu2020milliego}.
More importantly, both event cameras and mmWave radar feature \textit{millisecond latency} \cite{mmWaveUser}. These factors make mmWave a promising enhancement for event cameras in low-latency 3D object localization.
% Meanwhile, this fusion also holds potential in solving the issues of limited spatial resolution and scatter center drift faced by mmWave radar.

% mmWave signals, operating at high frequencies (30-300 GHz) with wide bandwidth, offer high sensing sensitivity. With fine-grained, directional sensing capability, mmWave sensing excels in object depth estimation. Both event cameras and mmWave radar share millisecond latency, making mmWave a promising enhancement for event cameras in low-latency 3D object localization. Additionally, this fusion can address the issues of limited spatial resolution and scatter center drift faced by mmWave radar.

% and resistance to weather and illumination conditions, 
% More importantly,尽管 mmWave 面临limited angular resolution和scatter center drift问题， both event cameras and mmWave radar share \textit{millisecond latency} \cite{mmWaveUser}, making mmWave a promising enhancement for event cameras in low-latency 3D object localization.
% Despite the issues of limited spatial resolution and scatter center drift faced by mmWave, both event cameras and mmWave radar share \textit{millisecond latency} \cite{mmWaveUser}. 
% This makes mmWave a promising enhancement for event cameras in low-latency 3D object localization, while the event camera also holds potential in solving mmWave radar issues.

% To better understand the potential of fusing the event camera and mmWave radar for low-latency and accurate localization, we conduct a benchmark study on landing drone localization at a real-world drone delivery airport (\fig \ref{relatedwork}a), as accurate and low-latency localization is essential for effective drone landing \cite{sun2023indoor}. 
% This is because landing is a critical phase where drones are most vulnerable \cite{wang2022micnest, xu2023taming, floreano2015science}, posing financial risks and safety threats \cite{Russiandrone}. 
% Higher accuracy improves landing success on designated platforms, while lower latency allows more reaction time to unexpected situations \cite{famili2022pilot, he2023acoustic, chi2022wi}.

To explore the potential of fusing the event camera and mmWave radar for improved 3D object localization, we conduct a benchmark study on drone localization during landing phase at a real-world drone delivery airport (\fig \ref{relatedwork}a). 
Accurate and low-latency localization is crucial for effective landing of the drone \cite{wang2022micnest, sun2023indoor}, as in this phase the drone is most vulnerable, posing financial risks and safety threats \cite{floreano2015science, Russiandrone}. 
Enhanced accuracy ensures successful landing on designated platforms, while reduced latency provides more reaction time for unexpected situations \cite{famili2022pilot, he2023acoustic, chi2022wi}.
Our benchmark study reveals that existing methods face fundamental challenges in 3D object localization, as elaborated below:

% \noindent $\bullet$ \textbf{C1: Millisecond sensing latency amplifies sensing noise, impairing drone detection.}
% \noindent $\bullet$ \textbf{C1: Differing noise distribution characteristics of both modalities hinder drone detection.}
% Unexpected environmental changes introduce irrelevant information as noise in sensing results \cite{xu2023taming}.
% Although both sensors have matched sensing latency, their noise distribution characteristics differ significantly due to their different mechanisms, hindering system's ability to identify signals changes caused by drone in both modalities \cite{zuo2024cross}, especially in millisecond latency (\fig \ref{relatedwork}b).
% However, traditional single modality-oriented noise filtering algorithms \cite{cao2024virteach, liu2024pmtrack, wang2021asynchronous, alzugaray2018asynchronous} achieve a low event and point cloud filtering rate (recall and precision < 65\% in \fig \ref{relatedwork}c) due to their rule-based pipelines struggle to distinguish drone-induced signal changes from scene dynamics.
% This results in detection precision bottlenecks, significantly diminishing the efficiency and accuracy of localization.

% 事件相机容易由于什么产生噪声，雷达容易由于什么产生噪声。对于同一个目标，这两种不同的传感器不仅产生异构的target-trigger的信息，也产生了空间上不同分布（dimentions，patterns）的噪声，而且这些噪声时间上也可能不同步，特别是在高时间分辨率的情况下。不幸的是，传统的方法要不就是针对单模态的滤波，要不就是对两个相似的信号进行滤波，不能应用到我们这个异构的高频场景下。
% Unexpected environmental changes introduce irrelevant information as noise in sensing results \cite{xu2023taming}.
% \noindent $\bullet$ \textbf{C1: Differing noise distribution characteristics of both modalities hinder drone detection.}
% Both sensor modalities yield not only heterogeneous information about the drone but also generate significantly heterogeneous noise. 
% Event cameras produce noise due to unexpected changes in brightness conditions, while mmWave radar struggles with noise caused by signal multipath effects.
% This noise differs greatly in dimensions and patterns, and it may lacks temporal synchronization, particularly under millisecond latency (\fig \ref{relatedwork}b). 
% These factors make noise filtering challenging, causing detection bottlenecks and reducing localization efficiency and accuracy \cite{xu2023taming}.
% Traditional noise filtering algorithms \cite{cao2024virteach, liu2024pmtrack, wang2021asynchronous, alzugaray2018asynchronous} target a specific modality, resulting in low noise event and point cloud filtering rates (recall and precision < 65\% in \fig \ref{relatedwork}c), limiting their effectiveness in our scenario.

% 一句背景，一句现象，一句结果，一句实验数据。
\noindent $\bullet$ \textbf{C1: Noise distribution characteristics of both modalities differ, hindering drone detection.}
% Both sensor modalities yield not only heterogeneous information about the drone but also generate significantly heterogeneous noise. 
These two sensor modalities not only provide different types of information but also generate significantly heterogeneous noise. 
Event cameras produce noise due to unexpected changes in brightness conditions, whereas mmWave radar struggles with noise caused by signal multipath effects.
These noises differ greatly in both dimension and pattern, which can also be asynchronous, especially under high temporal resolution (\fig \ref{relatedwork}b).
This spatial and temporal heterogeneity complicates noise filtering, causing detection bottlenecks \cite{xu2023taming}.
Unfortunately, existing traditional noise filtering algorithms \cite{cao2024virteach, liu2024pmtrack, wang2021asynchronous, alzugaray2018asynchronous} typically target a single modality, resulting in low noise event and point cloud filtering rates (recall and precision < 65\% in \fig \ref{relatedwork}c), limiting their effectiveness in our scenario.


% However, traditional noise filtering algorithms \cite{cao2024virteach, liu2024pmtrack, wang2021asynchronous, alzugaray2018asynchronous} are solely targeted at a specific modality and fail to exploit the consistency among different modalities, achieving a low event and point cloud filtering rate (recall and precision < 65\% in \fig \ref{relatedwork}c), which cannot be utilized in effective noise filtering in our scenario.
% This results in detection precision bottlenecks, significantly diminishing the efficiency and accuracy of localization.
% Although both sensors have matched sensing latency, their noise distribution characteristics differ significantly due to their different mechanisms, hindering system's ability to identify signals changes caused by drone in both modalities \cite{zuo2024cross}, especially in millisecond latency (\fig \ref{relatedwork}b).
% However, traditional single modality-oriented noise filtering algorithms \cite{cao2024virteach, liu2024pmtrack, wang2021asynchronous, alzugaray2018asynchronous} achieve a low event and point cloud filtering rate (recall and precision < 65\% in \fig \ref{relatedwork}c) due to their rule-based pipelines struggle to distinguish drone-induced signal changes from scene dynamics.

% \noindent $\bullet$ \textbf{C2: Ultra-large amount data burden the heterogeneous data fusion, delaying drone localization.}
% Once the drone is detected, accurate 3D spatial location estimation of it is essential, which is more time-consuming than detection due to additional processing (\eg, sensor fusion and optimization).
% The ultra-large amount of data generated by the millisecond latency further burdens the time consumption . 
% Although the localization accuracy is boosted, existing methods \cite{zhao20213d, falanga2020dynamic, mitrokhin2018event} introduces significant delays (\fig \ref{relatedwork}d).
% Moreover, asynchronous event streams and sparse point clouds from mmWave radar are heterogeneous in terms of precision, scale, and density. 
% Previous fusion methods (\eg, Extended kalman filter, particle filter, and graph optimization \cite{grisetti2010tutorial} in \fig \ref{relatedwork}d) suffer from severe cumulative drift error and lengthy processing latency, rendering them inadequate for accurate and low-latency localization.

\noindent $\bullet$ \textbf{C2: Ultra-large data volume burdens the heterogeneous data fusion, delaying drone localization.}
Accurately estimating 3D location of the drone after detection involves time-consuming processing steps, such as sensor fusion and optimization. 
% Once the drone is detected, we proceed to perform 3D localization on it.
% Accurately estimating 3D spatial location of drone involves several time-consuming processing steps, including the sensor fusion and optimization.
The ultra-large amount of data due to the high frequency further exacerbates the processing time, causing significant delays \cite{xu2021followupar}.
Meanwhile, the asynchronous event streams and sparse point clouds are heterogeneous in terms of precision, scale, and density, adding complexity to the sensor fusion.
Existing methods (\eg, Extended Kalman filter, particle filter, and graph optimization) suffer from cumulative drift error, heterogeneity issues, and lengthy processing latency, rendering them inadequate for accurate and low-latency localization as shown in \fig \ref{relatedwork}d \cite{zhao20213d, falanga2020dynamic, mitrokhin2018event, grisetti2010tutorial}.


\noindent \textbf{Our work.}
% We explore the sensing principles of the event camera and mmWave radar and propose EventLoc, an low latency-oriented event camera enhancement system that provides cm-level accurate 3D object localization with millisecond level latency to enable application of event camera in various 3D vision tasks.
We delve into the sensing principles of event cameras and mmWave radar, introducing EventLoc. 
This system enhances event camera functionality with a focus on low-latency 3D object localization, providing cm-level accuracy with millisecond latency on average. 
As a result, EventLoc broadens event camera application in diverse 3D vision tasks.
In detail, EventLoc features three key designs to fully unleash the potential of event camera and mmWave radar for 3D object localization, as elaborated below: \\
% and is implemented with adaptively acceleration algorithms to further improve accuracy and reduce latency, 
\noindent $\bullet$ \textbf{On system architecture front.}
By incorporating mmWave radar with millisecond latency, we enhance the performance of event camera and improve 3D localization performance at the data source.
EventLoc features a carefully designed system architecture that tightly couples event camera and mmWave radar. 
This integration spans from early-stage filtering to later-stage fusion and optimization, fully leveraging the unique advantages of both sensors (§\ref{3.2}). \\
\noindent $\bullet$ \textbf{On system algorithm front.}
We first introduce the Consi-stency-Instructed Collaborative Tracking (\textit{CCT}) algorithm to extract \textit{consistent information} in sensing data from both modalities to filter out environment-triggered noise with a low false positive rate, enhancing the detection performance with a low-latency (§\ref{4.1}). 
We then present the Graph-Informed Adaptive Joint Optimization (\textit{GAJO}) algorithm to fully fuse \textit{complementary information} from both modalities, accelerating the optimization in localizing the object (§\ref{4.2}). \\
\noindent $\bullet$ \textbf{On system implementation front.}
We further analyze the sources of latency and propose an Adaptive Optimization method for boosting the \textit{GAJO}. 
This method dynamically optimizes the set of locations rather than relying on a fixed sliding window, further enhancing the accuracy of localization and reducing latency (§\ref{5.1}).

\begin{figure*}[t]
    \setlength{\abovecaptionskip}{0.4cm} % height above Figure X caption
    \setlength{\belowcaptionskip}{-0.5cm}
    \setlength{\subfigcapskip}{-0.25cm}
    \centering
        \includegraphics[width=2\columnwidth]{Figs/overview2.png}
        \vspace{-0.2cm}
    \caption{System architecture of EventLoc.}
    \label{overview}
    % \vspace{-0.2cm}
\end{figure*} 

\noindent \textbf{Evaluation and Result.} 
We fully implement EventLoc with COTS event camera and mmWave radar.
Extensive experiments in indoor/outdoor environments are conducted with different drone flight conditions to comprehensively evaluate performance of EventLoc.
We compare the end-to-end drone localization accuracy and latency of EventLoc with three SOTA methods.
% Through over 30 hours of real-world experiments, we demonstrate that EventLoc enhances event camera with mmWave radar by achieving a localization accuracy of 1.01 $dm$, surpassing all baselines by >50\%. EventLoc further achieves localization latency of 5.15 $ms$, outperforming baselines by >50\% in average.
Through over 30 hours of experiments, we demonstrate that EventLoc enhances event camera with mmWave radar by achieving an average localization accuracy of 0.101 $m$ and latency of 5.15 $ms$, surpassing all baselines by >50\% on average.
Additionally, EventLoc is marginally affected by factors such as drone type and envir. conditions.\\
\textbf{Real-world deployment.}
We have deployed the sensor platform with EventLoc at a real-world drone delivery airport as shown in \fig \ref{relatedwork}a to demonstrate practicability of the system.
10 hours study shows that EventLoc meets drone landing demands within the constraints of available resources.

\noindent \textbf{Contributions.} This paper makes following contributions.

\noindent $(1)$ We propose EventLoc, a novel low latency-oriented event camera enhancement system. It tightly integrates asynchronous events and mmWave radar sparse point clouds, achieving accurate drone localization with millisecond latency.\\
\noindent $(2)$ We propose the $CCT$, a light-weight cross-modal noise filter to push the limit of detection accuracy by leveraging the \textit{consistent information} from both modalities. \\
\noindent $(3)$  We propose the $GAJO$, a factor graph-based optimization framework that fully harnessing \textit{complementary information} from both modalities to enhance localization performance.\\
% accuracy and latency
\noindent $(4)$ We implement and extensively evaluate EventLoc by comparing it with three SOTA methods, showing its effectiveness. We also deploy EventLoc in a real-world drone delivery airport, demonstrating feasibility of EventLoc.
% The remainder of the paper is organized as follows:
% §2 provides an overview of EventLoc, with detailed descriptions of the Consistency-Instructed Collaborative Tracking algorithm in §3.1 and the Graph-Informed Adaptive Joint Optimization algorithm in §3.2. §4 showcases the adaptive acceleration algorithms and implementation. §5 details our extensive indoor and outdoor experiments with EventLoc. §6 presents our experiments conducted at a real-world delivery airport. §7 discusses related work. §8 concludes the paper.

